Mechanising Denotational Semantics in Agda

Mechanisation of a mathematical definition (also referred to as formalisation) has many benefits. Here, we focus on mechanising denotational semantic definitions of programming languages by embedding them in the Agda language. The Agda type-checker detects and reports any issues with the wellformedness and type correctness of the embedded definitions. To minimise the effort required, and to facilitate correlation of the original definition with its Agda embedding, mechanisation should not involve significant reformulation or extension. Here, we show how to embed conventional Scott-Strachey denotational definitions in Agda with almost no changes to $\lambda$-notation or domain equations. Agda notation for definitions of types and functions corresponds closely to the conventional meta-notation of denotational semantics. We have developed a collection of Agda modules with postulated types for commonly used domain constructors and their associated operations. We illustrate our approach with mechanisations of three denotational definitions: a model of the untyped $\lambda$-calculus, Plotkin's denotational semantics of PCF, and a semantics of a sublanguage of Scheme. In previous work, similar mechanisations in Agda have revealed several unsuspected wellformedness issues in published denotational definitions. Some of the postulated properties of our definitions are inconsistent with a classical set-theoretic interpretation of Agda. We conjecture that they would be consistent with an interpretation of Agda in a higher-order intuititionistic logic, such as that used by Simpson in his work on synthetic domain theory. After recalling previous work on mechanising domain theory, we consider the possibility of mechanising synthetic domain theory in Agda.

==> generated/Properties/Domains.tex <==
\subsection{Domains}\label{Properties/Domains-domains}
%
\begin{AgdaSuppressSpace}
\begin{code}[hide]%
\>[0]\AgdaSymbol{\{-\#}\AgdaSpace{}%
\AgdaKeyword{OPTIONS}\AgdaSpace{}%
\AgdaPragma{--rewriting}\AgdaSpace{}%
\AgdaPragma{--confluence-check}\AgdaSpace{}%
\AgdaSymbol{\#-\}}\<%
\\
\>[0]\<%
\end{code}
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
%
%<*AgdaTag-Properties.Domains>
\AgdaModule{Properties.Domains}%
%</AgdaTag-Properties.Domains>
\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
%
%<*AgdaTag-Notation.Domains>
\AgdaModule{Notation.Domains}%
%</AgdaTag-Notation.Domains>
\AgdaSpace{}%
\AgdaKeyword{public}\<%
\end{code}
\end{AgdaSuppressSpace}


==> generated/Properties/Flat/Booleans.tex <==
\subsubsection{Booleans}\label{Properties/Flat/Booleans-booleans}
%
\begin{AgdaSuppressSpace}
\begin{code}[hide]%
\>[0]\AgdaSymbol{\{-\#}\AgdaSpace{}%
\AgdaKeyword{OPTIONS}\AgdaSpace{}%
\AgdaPragma{--rewriting}\AgdaSpace{}%
\AgdaPragma{--confluence-check}\AgdaSpace{}%
\AgdaSymbol{\#-\}}\<%
\\
\>[0]\<%
\end{code}
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
%
%<*AgdaTag-Properties.Flat.Booleans>
\AgdaModule{Properties.Flat.Booleans}%
%</AgdaTag-Properties.Flat.Booleans>
\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
%
%<*AgdaTag-Notation.Flat.Booleans>
\AgdaModule{Notation.Flat.Booleans}%
%</AgdaTag-Notation.Flat.Booleans>
\AgdaSpace{}%
\AgdaKeyword{public}\<%
\end{code}
\end{AgdaSuppressSpace}


==> generated/Properties/Flat/Naturals.tex <==
\subsubsection{Naturals}\label{Properties/Flat/Naturals-naturals}
%
\begin{AgdaSuppressSpace}
\begin{code}[hide]%
\>[0]\AgdaSymbol{\{-\#}\AgdaSpace{}%
\AgdaKeyword{OPTIONS}\AgdaSpace{}%
\AgdaPragma{--rewriting}\AgdaSpace{}%
\AgdaPragma{--confluence-check}\AgdaSpace{}%
\AgdaSymbol{\#-\}}\<%
\\
\>[0]\<%
\end{code}
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
%
%<*AgdaTag-Properties.Flat.Naturals>
\AgdaModule{Properties.Flat.Naturals}%
%</AgdaTag-Properties.Flat.Naturals>
\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
%
%<*AgdaTag-Notation.Flat.Naturals>
\AgdaModule{Notation.Flat.Naturals}%
%</AgdaTag-Notation.Flat.Naturals>
\AgdaSpace{}%
\AgdaKeyword{public}\<%
\end{code}
\end{AgdaSuppressSpace}


==> generated/Properties/Products.tex <==
\subsection{Product Domains}\label{Properties/Products-product-domains}
%
\begin{AgdaSuppressSpace}
\begin{code}[hide]%
\>[0]\AgdaSymbol{\{-\#}\AgdaSpace{}%
\AgdaKeyword{OPTIONS}\AgdaSpace{}%
\AgdaPragma{--rewriting}\AgdaSpace{}%
\AgdaPragma{--confluence-check}\AgdaSpace{}%
\AgdaPragma{--lossy-unification}\AgdaSpace{}%
\AgdaSymbol{\#-\}}\<%
\\
\>[0]\<%
\end{code}
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
%
%<*AgdaTag-Properties.Products>
\AgdaModule{Properties.Products}%
%</AgdaTag-Properties.Products>
\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
%
%<*AgdaTag-Notation.Domains>
\AgdaModule{Notation.Domains}%
%</AgdaTag-Notation.Domains>
\<%
\\
%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
%
%<*AgdaTag-Notation.Functions>
\AgdaModule{Notation.Functions}%
%</AgdaTag-Notation.Functions>
\<%
\\
%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
%
%<*AgdaTag-Notation.Products>
\AgdaModule{Notation.Products}%
%</AgdaTag-Notation.Products>
\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{%
%<*AgdaTag-\AgdaUnderscore{>
\AgdaPostulate{\AgdaUnderscore{}%
%</AgdaTag-\AgdaUnderscore{>
×\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-\AgdaUnderscore{>
\AgdaPostulate{\AgdaUnderscore{}%
%</AgdaTag-\AgdaUnderscore{>
,\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-\AgdaUnderscore{>
\AgdaPostulate{\AgdaUnderscore{}%
%</AgdaTag-\AgdaUnderscore{>
↓₁}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-\AgdaUnderscore{>
\AgdaPostulate{\AgdaUnderscore{}%
%</AgdaTag-\AgdaUnderscore{>
↓₂}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{public}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{δ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟪>
\AgdaPostulate{⟪}%
%</AgdaTag-⟪>
}\AgdaSpace{}%
\AgdaGeneralizable{D}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟫>
\AgdaPostulate{⟫}%
%</AgdaTag-⟫>
}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaGeneralizable{ε}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟪>
\AgdaPostulate{⟪}%
%</AgdaTag-⟪>
}\AgdaSpace{}%
\AgdaGeneralizable{E}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟫>
\AgdaPostulate{⟫}%
%</AgdaTag-⟫>
}\<%
\\
%
\>[2]\AgdaKeyword{postulate}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]%
%<*AgdaTag-elim-↓₁>
\AgdaPostulate{elim-↓₁}%
%</AgdaTag-elim-↓₁>
%
\>[14]\AgdaSymbol{:}%
\>[17]\AgdaSymbol{(}\AgdaSpace{}%
\AgdaGeneralizable{δ}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-,>
\AgdaPostulate{,}%
%</AgdaTag-,>
}\AgdaSpace{}%
\AgdaGeneralizable{ε}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-↓₁>
\AgdaPostulate{↓₁}%
%</AgdaTag-↓₁>
}%
\>[34]\AgdaOperator{%
%<*AgdaTag-≡>
\AgdaDatatype{≡}%
%</AgdaTag-≡>
}%
\>[37]\AgdaGeneralizable{δ}\<%
\\
%
\>[4]%
%<*AgdaTag-elim-↓₂>
\AgdaPostulate{elim-↓₂}%
%</AgdaTag-elim-↓₂>
%
\>[14]\AgdaSymbol{:}%
\>[17]\AgdaSymbol{(}\AgdaSpace{}%
\AgdaGeneralizable{δ}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-,>
\AgdaPostulate{,}%
%</AgdaTag-,>
}\AgdaSpace{}%
\AgdaGeneralizable{ε}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-↓₂>
\AgdaPostulate{↓₂}%
%</AgdaTag-↓₂>
}%
\>[34]\AgdaOperator{%
%<*AgdaTag-≡>
\AgdaDatatype{≡}%
%</AgdaTag-≡>
}%
\>[37]\AgdaGeneralizable{ε}\<%
\\
%
\>[4]%
%<*AgdaTag-elim-⊥-⊥>
\AgdaPostulate{elim-⊥-⊥}%
%</AgdaTag-elim-⊥-⊥>
%
\>[14]\AgdaSymbol{:}%
\>[17]\AgdaSymbol{(}\AgdaSpace{}%
%
%<*AgdaTag-⊥>
\AgdaPostulate{⊥}%
%</AgdaTag-⊥>
\AgdaSymbol{\{}\AgdaGeneralizable{D}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-,>
\AgdaPostulate{,}%
%</AgdaTag-,>
}\AgdaSpace{}%
%
%<*AgdaTag-⊥>
\AgdaPostulate{⊥}%
%</AgdaTag-⊥>
\AgdaSymbol{\{}\AgdaGeneralizable{E}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{)}%
\>[34]\AgdaOperator{%
%<*AgdaTag-≡>
\AgdaDatatype{≡}%
%</AgdaTag-≡>
}%
\>[37]%
%<*AgdaTag-⊥>
\AgdaPostulate{⊥}%
%</AgdaTag-⊥>
\AgdaSymbol{\{}\AgdaGeneralizable{D}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-×>
\AgdaPostulate{×}%
%</AgdaTag-×>
}\AgdaSpace{}%
\AgdaGeneralizable{E}\AgdaSymbol{\}}\<%
\\
%
\>[2]\AgdaSymbol{\{-\#}\AgdaSpace{}%
\AgdaKeyword{REWRITE}\AgdaSpace{}%
%
%<*AgdaTag-elim-↓₁>
\AgdaPostulate{elim-↓₁}%
%</AgdaTag-elim-↓₁>
\AgdaSpace{}%
%
%<*AgdaTag-elim-↓₂>
\AgdaPostulate{elim-↓₂}%
%</AgdaTag-elim-↓₂>
\AgdaSpace{}%
\AgdaSymbol{\#-\}}\<%
\end{code}
\end{AgdaSuppressSpace}


==> generated/Properties/Products/Sequences.tex <==
\subsubsection{Sequences}\label{Properties/Products/Sequences-sequences}
%
\begin{AgdaSuppressSpace}
\begin{code}[hide]%
\>[0]\AgdaSymbol{\{-\#}\AgdaSpace{}%
\AgdaKeyword{OPTIONS}\AgdaSpace{}%
\AgdaPragma{--rewriting}\AgdaSpace{}%
\AgdaPragma{--confluence-check}\AgdaSpace{}%
\AgdaSymbol{\#-\}}\<%
\\
\>[0]\<%
\end{code}
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
%
%<*AgdaTag-Properties.Products.Sequences>
\AgdaModule{Properties.Products.Sequences}%
%</AgdaTag-Properties.Products.Sequences>
\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
%
%<*AgdaTag-Notation.Products.Sequences>
\AgdaModule{Notation.Products.Sequences}%
%</AgdaTag-Notation.Products.Sequences>
\AgdaSpace{}%
\AgdaKeyword{public}\<%
\end{code}
\end{AgdaSuppressSpace}


==> generated/Properties/Products/Tuples.tex <==
\subsubsection{Tuples}\label{Properties/Products/Tuples-tuples}
%
\begin{AgdaSuppressSpace}
\begin{code}[hide]%
\>[0]\AgdaSymbol{\{-\#}\AgdaSpace{}%
\AgdaKeyword{OPTIONS}\AgdaSpace{}%
\AgdaPragma{--rewriting}\AgdaSpace{}%
\AgdaPragma{--confluence-check}\AgdaSpace{}%
\AgdaSymbol{\#-\}}\<%
\\
\>[0]\<%
\end{code}
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
%
%<*AgdaTag-Properties.Products.Tuples>
\AgdaModule{Properties.Products.Tuples}%
%</AgdaTag-Properties.Products.Tuples>
\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
%
%<*AgdaTag-Notation.Products.Tuples>
\AgdaModule{Notation.Products.Tuples}%
%</AgdaTag-Notation.Products.Tuples>
\AgdaSpace{}%
\AgdaKeyword{public}\<%
\end{code}
\end{AgdaSuppressSpace}


==> generated/Properties/Sums.tex <==
\subsection{Sum Domains}\label{Properties/Sums-sum-domains}
%
\begin{AgdaSuppressSpace}
\begin{code}[hide]%
\>[0]\AgdaSymbol{\{-\#}\AgdaSpace{}%
\AgdaKeyword{OPTIONS}\AgdaSpace{}%
\AgdaPragma{--rewriting}\AgdaSpace{}%
\AgdaPragma{--confluence-check}\AgdaSpace{}%
\AgdaPragma{--lossy-unification}\AgdaSpace{}%
\AgdaSymbol{\#-\}}\<%
\\
\>[0]\<%
\end{code}
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
%
%<*AgdaTag-Properties.Sums>
\AgdaModule{Properties.Sums}%
%</AgdaTag-Properties.Sums>
\AgdaSpace{}%
\AgdaKeyword{where}\<%
\end{code}
\begin{code}[hide]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
%
%<*AgdaTag-Notation.Domains>
\AgdaModule{Notation.Domains}%
%</AgdaTag-Notation.Domains>
\<%
\\
%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
%
%<*AgdaTag-Notation.Functions>
\AgdaModule{Notation.Functions}%
%</AgdaTag-Notation.Functions>
\<%
\\
%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
%
%<*AgdaTag-Notation.Sums>
\AgdaModule{Notation.Sums}%
%</AgdaTag-Notation.Sums>
\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{%
%<*AgdaTag-\AgdaUnderscore{>
\AgdaPostulate{\AgdaUnderscore{}%
%</AgdaTag-\AgdaUnderscore{>
+\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
%
%<*AgdaTag-inj₁>
\AgdaPostulate{inj₁}%
%</AgdaTag-inj₁>
\AgdaSymbol{;}\AgdaSpace{}%
%
%<*AgdaTag-inj₂>
\AgdaPostulate{inj₂}%
%</AgdaTag-inj₂>
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-[\AgdaUnderscore{>
\AgdaPostulate{[\AgdaUnderscore{}%
%</AgdaTag-[\AgdaUnderscore{>
,\AgdaUnderscore{}]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{public}\<%
\end{code}
\begin{code}%
\>[0]\<%
\\
%
\>[2]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟪>
\AgdaPostulate{⟪}%
%</AgdaTag-⟪>
}\AgdaSpace{}%
\AgdaGeneralizable{D}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-→ᶜ>
\AgdaPostulate{→ᶜ}%
%</AgdaTag-→ᶜ>
}\AgdaSpace{}%
\AgdaGeneralizable{F}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟫>
\AgdaPostulate{⟫}%
%</AgdaTag-⟫>
}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaGeneralizable{ψ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟪>
\AgdaPostulate{⟪}%
%</AgdaTag-⟪>
}\AgdaSpace{}%
\AgdaGeneralizable{E}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-→ᶜ>
\AgdaPostulate{→ᶜ}%
%</AgdaTag-→ᶜ>
}\AgdaSpace{}%
\AgdaGeneralizable{F}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟫>
\AgdaPostulate{⟫}%
%</AgdaTag-⟫>
}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaGeneralizable{δ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟪>
\AgdaPostulate{⟪}%
%</AgdaTag-⟪>
}\AgdaSpace{}%
\AgdaGeneralizable{D}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟫>
\AgdaPostulate{⟫}%
%</AgdaTag-⟫>
}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaGeneralizable{ε}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟪>
\AgdaPostulate{⟪}%
%</AgdaTag-⟪>
}\AgdaSpace{}%
\AgdaGeneralizable{E}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟫>
\AgdaPostulate{⟫}%
%</AgdaTag-⟫>
}\<%
\\
%
\>[2]\AgdaKeyword{postulate}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]%
%<*AgdaTag-elim-inj₁>
\AgdaPostulate{elim-inj₁}%
%</AgdaTag-elim-inj₁>
%
\>[15]\AgdaSymbol{:}%
\>[18]\AgdaOperator{%
%<*AgdaTag-[>
\AgdaPostulate{[}%
%</AgdaTag-[>
}\AgdaSpace{}%
\AgdaGeneralizable{φ}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-,>
\AgdaPostulate{,}%
%</AgdaTag-,>
}\AgdaSpace{}%
\AgdaGeneralizable{ψ}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-]>
\AgdaPostulate{]}%
%</AgdaTag-]>
}\AgdaSpace{}%
\AgdaSymbol{(}%
%<*AgdaTag-inj₁>
\AgdaPostulate{inj₁}%
%</AgdaTag-inj₁>
\AgdaSpace{}%
\AgdaGeneralizable{δ}\AgdaSymbol{)}%
\>[38]\AgdaOperator{%
%<*AgdaTag-≡>
\AgdaDatatype{≡}%
%</AgdaTag-≡>
}%
\>[41]\AgdaGeneralizable{φ}\AgdaSpace{}%
\AgdaGeneralizable{δ}\<%
\\
%
\>[4]%
%<*AgdaTag-elim-inj₂>
\AgdaPostulate{elim-inj₂}%
%</AgdaTag-elim-inj₂>
%
\>[15]\AgdaSymbol{:}%
\>[18]\AgdaOperator{%
%<*AgdaTag-[>
\AgdaPostulate{[}%
%</AgdaTag-[>
}\AgdaSpace{}%
\AgdaGeneralizable{φ}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-,>
\AgdaPostulate{,}%
%</AgdaTag-,>
}\AgdaSpace{}%
\AgdaGeneralizable{ψ}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-]>
\AgdaPostulate{]}%
%</AgdaTag-]>
}\AgdaSpace{}%
\AgdaSymbol{(}%
%<*AgdaTag-inj₂>
\AgdaPostulate{inj₂}%
%</AgdaTag-inj₂>
\AgdaSpace{}%
\AgdaGeneralizable{ε}\AgdaSymbol{)}%
\>[38]\AgdaOperator{%
%<*AgdaTag-≡>
\AgdaDatatype{≡}%
%</AgdaTag-≡>
}%
\>[41]\AgdaGeneralizable{ψ}\AgdaSpace{}%
\AgdaGeneralizable{ε}\<%
\\
%
\>[4]%
%<*AgdaTag-elim-[]-⊥>
\AgdaPostulate{elim-[]-⊥}%
%</AgdaTag-elim-[]-⊥>
%
\>[15]\AgdaSymbol{:}%
\>[18]\AgdaOperator{%
%<*AgdaTag-[>
\AgdaPostulate{[}%
%</AgdaTag-[>
}\AgdaSpace{}%
\AgdaGeneralizable{φ}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-,>
\AgdaPostulate{,}%
%</AgdaTag-,>
}\AgdaSpace{}%
\AgdaGeneralizable{ψ}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-]>
\AgdaPostulate{]}%
%</AgdaTag-]>
}\AgdaSpace{}%
%
%<*AgdaTag-⊥>
\AgdaPostulate{⊥}%
%</AgdaTag-⊥>
%
\>[38]\AgdaOperator{%
%<*AgdaTag-≡>
\AgdaDatatype{≡}%
%</AgdaTag-≡>
}%
\>[41]%
%<*AgdaTag-⊥>
\AgdaPostulate{⊥}%
%</AgdaTag-⊥>
\<%
\\
%
\>[2]\AgdaSymbol{\{-\#}\AgdaSpace{}%
\AgdaKeyword{REWRITE}\AgdaSpace{}%
%
%<*AgdaTag-elim-inj₁>
\AgdaPostulate{elim-inj₁}%
%</AgdaTag-elim-inj₁>
\AgdaSpace{}%
%
%<*AgdaTag-elim-inj₂>
\AgdaPostulate{elim-inj₂}%
%</AgdaTag-elim-inj₂>
\AgdaSpace{}%
\AgdaSymbol{\#-\}}\<%
\\
\>[0]\<%
\end{code}
\begin{code}[hide]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
%
%<*AgdaTag-Notation.Sums>
\AgdaModule{Notation.Sums}%
%</AgdaTag-Notation.Sums>
\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{n}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-\AgdaUnderscore{>
\AgdaPostulate{\AgdaUnderscore{}%
%</AgdaTag-\AgdaUnderscore{>
≳\AgdaUnderscore{}↦\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-\AgdaUnderscore{>
\AgdaPostulate{\AgdaUnderscore{}%
%</AgdaTag-\AgdaUnderscore{>
in⊥\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-\AgdaUnderscore{>
\AgdaPostulate{\AgdaUnderscore{}%
%</AgdaTag-\AgdaUnderscore{>
|⊥\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-\AgdaUnderscore{>
\AgdaPostulate{\AgdaUnderscore{}%
%</AgdaTag-\AgdaUnderscore{>
∈⊥\AgdaUnderscore{}}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{public}\<%
\\
%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
%
%<*AgdaTag-Notation.Flat>
\AgdaModule{Notation.Flat}%
%</AgdaTag-Notation.Flat>
\<%
\\
%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
%
%<*AgdaTag-Notation.Flat.Booleans>
\AgdaModule{Notation.Flat.Booleans}%
%</AgdaTag-Notation.Flat.Booleans>
\<%
\\
%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
%
%<*AgdaTag-Notation.Flat.Naturals>
\AgdaModule{Notation.Flat.Naturals}%
%</AgdaTag-Notation.Flat.Naturals>
\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
%
%<*AgdaTag-Relation.Binary.PropositionalEquality.Core>
\AgdaModule{Relation.Binary.PropositionalEquality.Core}%
%</AgdaTag-Relation.Binary.PropositionalEquality.Core>
\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{%
%<*AgdaTag-\AgdaUnderscore{>
\AgdaFunction{\AgdaUnderscore{}%
%</AgdaTag-\AgdaUnderscore{>
≢\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\end{code}
\begin{code}%
%
\>[2]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{D′}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
%
%<*AgdaTag-Domain>
\AgdaPostulate{Domain}%
%</AgdaTag-Domain>
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaGeneralizable{n′}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
%
%<*AgdaTag-Nat>
\AgdaDatatype{Nat}%
%</AgdaTag-Nat>
\<%
\\
%
\>[2]\AgdaKeyword{postulate}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]%
%<*AgdaTag-elim-∈⊥>
\AgdaPostulate{elim-∈⊥}%
%</AgdaTag-elim-∈⊥>
%
\>[15]\AgdaSymbol{:}%
\>[18]\AgdaSymbol{\{\{}\AgdaBound{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{E}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-≳>
\AgdaPostulate{≳}%
%</AgdaTag-≳>
}\AgdaSpace{}%
\AgdaGeneralizable{n}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-↦>
\AgdaPostulate{↦}%
%</AgdaTag-↦>
}\AgdaSpace{}%
\AgdaGeneralizable{D}\AgdaSymbol{\}\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{\{\{}\AgdaBound{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{E}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-≳>
\AgdaPostulate{≳}%
%</AgdaTag-≳>
}\AgdaSpace{}%
\AgdaGeneralizable{n′}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-↦>
\AgdaPostulate{↦}%
%</AgdaTag-↦>
}\AgdaSpace{}%
\AgdaGeneralizable{D′}\AgdaSymbol{\}\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{δ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟪>
\AgdaPostulate{⟪}%
%</AgdaTag-⟪>
}\AgdaSpace{}%
\AgdaGeneralizable{D}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟫>
\AgdaPostulate{⟫}%
%</AgdaTag-⟫>
}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
%
\>[18]\AgdaSymbol{(}\AgdaBound{δ}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-in⊥>
\AgdaPostulate{in⊥}%
%</AgdaTag-in⊥>
}\AgdaSpace{}%
\AgdaGeneralizable{E}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-∈⊥>
\AgdaPostulate{∈⊥}%
%</AgdaTag-∈⊥>
}\AgdaSpace{}%
\AgdaGeneralizable{D′}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-≡>
\AgdaDatatype{≡}%
%</AgdaTag-≡>
}\AgdaSpace{}%
%
%<*AgdaTag-↑>
\AgdaPostulate{↑}%
%</AgdaTag-↑>
\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{n}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{==ᴺ}}\AgdaSpace{}%
\AgdaGeneralizable{n′}\AgdaSymbol{)}\<%
\\
%
\>[4]%
%<*AgdaTag-elim-|⊥>
\AgdaPostulate{elim-|⊥}%
%</AgdaTag-elim-|⊥>
%
\>[15]\AgdaSymbol{:}%
\>[18]\AgdaSymbol{\{\{}\AgdaBound{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{E}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-≳>
\AgdaPostulate{≳}%
%</AgdaTag-≳>
}\AgdaSpace{}%
\AgdaGeneralizable{n}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-↦>
\AgdaPostulate{↦}%
%</AgdaTag-↦>
}\AgdaSpace{}%
\AgdaGeneralizable{D}\AgdaSymbol{\}\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{δ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟪>
\AgdaPostulate{⟪}%
%</AgdaTag-⟪>
}\AgdaSpace{}%
\AgdaGeneralizable{D}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟫>
\AgdaPostulate{⟫}%
%</AgdaTag-⟫>
}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{δ}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-in⊥>
\AgdaPostulate{in⊥}%
%</AgdaTag-in⊥>
}\AgdaSpace{}%
\AgdaGeneralizable{E}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-|⊥>
\AgdaPostulate{|⊥}%
%</AgdaTag-|⊥>
}\AgdaSpace{}%
\AgdaGeneralizable{D}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-≡>
\AgdaDatatype{≡}%
%</AgdaTag-≡>
}\AgdaSpace{}%
\AgdaBound{δ}\<%
\\
%
\>[4]%
%<*AgdaTag-elim-∈⊥-⊥>
\AgdaPostulate{elim-∈⊥-⊥}%
%</AgdaTag-elim-∈⊥-⊥>
%
\>[15]\AgdaSymbol{:}%
\>[18]\AgdaSymbol{\{\{}\AgdaBound{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{E}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-≳>
\AgdaPostulate{≳}%
%</AgdaTag-≳>
}\AgdaSpace{}%
\AgdaGeneralizable{n}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-↦>
\AgdaPostulate{↦}%
%</AgdaTag-↦>
}\AgdaSpace{}%
\AgdaGeneralizable{D}\AgdaSymbol{\}\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{\{\{}\AgdaBound{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{E}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-≳>
\AgdaPostulate{≳}%
%</AgdaTag-≳>
}\AgdaSpace{}%
\AgdaGeneralizable{n′}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-↦>
\AgdaPostulate{↦}%
%</AgdaTag-↦>
}\AgdaSpace{}%
\AgdaGeneralizable{D′}\AgdaSymbol{\}\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{δ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟪>
\AgdaPostulate{⟪}%
%</AgdaTag-⟪>
}\AgdaSpace{}%
\AgdaGeneralizable{D}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-⟫>
\AgdaPostulate{⟫}%
%</AgdaTag-⟫>
}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
%
\>[18]\AgdaSymbol{\{}\AgdaGeneralizable{n}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-≢>
\AgdaFunction{≢}%
%</AgdaTag-≢>
}\AgdaSpace{}%
\AgdaGeneralizable{n′}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{δ}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-in⊥>
\AgdaPostulate{in⊥}%
%</AgdaTag-in⊥>
}\AgdaSpace{}%
\AgdaGeneralizable{E}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-|⊥>
\AgdaPostulate{|⊥}%
%</AgdaTag-|⊥>
}\AgdaSpace{}%
\AgdaGeneralizable{D′}\AgdaSpace{}%
\AgdaOperator{%
%<*AgdaTag-≡>
\AgdaDatatype{≡}%
%</AgdaTag-≡>
}\AgdaSpace{}%
%
%<*AgdaTag-⊥>
\AgdaPostulate{⊥}%
%</AgdaTag-⊥>
\<%
\\
%
\>[2]\AgdaSymbol{\{-\#}\AgdaSpace{}%
\AgdaKeyword{REWRITE}\AgdaSpace{}%
%
%<*AgdaTag-elim-∈⊥>
\AgdaPostulate{elim-∈⊥}%
%</AgdaTag-elim-∈⊥>
\AgdaSpace{}%
%
%<*AgdaTag-elim-|⊥>
\AgdaPostulate{elim-|⊥}%
%</AgdaTag-elim-|⊥>
\AgdaSpace{}%
\AgdaSymbol{\#-\}}\<%
\end{code}
\end{AgdaSuppressSpace}


==> generated/Properties/Updates.tex <==
\subsection{Updates}\label{Properties/Updates-updates}
%
\begin{AgdaSuppressSpace}
\begin{code}[hide]%
\>[0]\AgdaSymbol{\{-\#}\AgdaSpace{}%
\AgdaKeyword{OPTIONS}\AgdaSpace{}%
\AgdaPragma{--rewriting}\AgdaSpace{}%
\AgdaPragma{--confluence-check}\AgdaSpace{}%
\AgdaSymbol{\#-\}}\<%
\\
\>[0]\<%
\end{code}
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
%
%<*AgdaTag-Properties.Updates>
\AgdaModule{Properties.Updates}%
%</AgdaTag-Properties.Updates>
\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
%
%<*AgdaTag-Notation.Updates>
\AgdaModule{Notation.Updates}%
%</AgdaTag-Notation.Updates>
\AgdaSpace{}%
\AgdaKeyword{public}\<%
\end{code}
\end{AgdaSuppressSpace}

